An Empirical Comparison of Big Graph Frameworks in the Context of Network Analysis

Complex networks are relational data sets commonly represented as graphs. The analysis of their intricate structure is relevant to many areas of science and commerce, and data sets may reach sizes that require distributed storage and processing. We describe and compare programming models for distributed computing with a focus on graph algorithms for large-scale complex network analysis. Four frameworks - GraphLab, Apache Giraph, Giraph++ and Apache Flink - are used to implement algorithms for the representative problems Connected Components, Community Detection, PageRank and Clustering Coefficients. The implementations are executed on a computer cluster to evaluate the frameworks' suitability in practice and to compare their performance to that of the single-machine, shared-memory parallel network analysis package NetworKit. Out of the distributed frameworks, GraphLab and Apache Giraph generally show the best performance. In our experiments a cluster of eight computers running Apache Giraph enables the analysis of a network with about 2 billion edges, which is too large for a single machine of the same type. However, for networks that fit into memory of one machine, the performance of the shared-memory parallel implementation is far better than the distributed ones. The study provides experimental evidence for selecting the appropriate framework depending on the task and data volume.

==> codes/ch02_gas_model.tex <==
\begin{algorithm}
  \caption[General GAS program execution]{GAS program pseudo code, based on \cite{graphlabDocumentation}}\label{alg:gas_program}
  \SetKwFunction{gas}{GAS\_Program}
  \SetKwFunction{parallel}{Parallel}

	\gas{vertex}
	\Begin{
		gather\_result $\leftarrow$ 0\tcc*[r]{Gather}
		\parallel \ForEach{edge $\in$ vertex.edges}{
			edge\_information $\leftarrow$ gather(vertex, edge)\;
			gather\_result $\leftarrow$ gather\_sum(gather\_result, edge\_information)\;
		}
		 apply(vertex, gather\_result)\tcc*[r]{Apply}
		\parallel \ForEach{edge $\in$ vertex.edges}{
			scatter(vertex, edge)\tcc*[r]{Scatter}
		}
	}
\end{algorithm}

==> codes/ch02_gas_pregel_emulation.tex <==
\begin{algorithm}[h]
\SetKwData{messagePuffer}{messagePuffer}


\gather{\Vertex, \Edge}
\Begin{
	\KwRet{\Edge.\messages}
}
\gathersum{v1, v2}
\Begin{
	\tcp{append all messages}
	\KwRet{\append{v1, v2}}
}
\apply{vertex, messages}
\Begin{
	\tcp{contains code of the Pregel compute function
	\\edge data can be derived from the incoming messages
	\\messages can be sent using sendMessage() implemented below}
	PregelCompute()\;
}
\sendmsg{receiver, message}
\Begin{
	messagePuffer.add(receiver, message);
}
\scatter{\Vertex, \Edge}
\Begin{
	\messages $\leftarrow$ \messagePuffer.get(\Edge.target.id)\;
	\Edge.\messages $\leftarrow$ \messages\;
	\If{\messages.size > 0}{
		\signal(\Edge.target.id)\;
	}
}
\caption{Emulation of a Pregel program in GAS}
\label{alg:gas_pregel_emulation}
\end{algorithm}

==> codes/ch02_mapreduce_pagerank.tex <==
\begin{algorithm}
  \caption[PageRank in MapReduce]{PageRank in MapReduce \citep{LinTextProcessing}}
  \label{alg:mapreduce_pagerank}
  \SetKwData{rank}{RANK}
  \SetKwData{vertex}{VERTEX}

	\map{vertexId, vertex}
	\Begin{
		Emit(vertexId, \vertex vertex)\;
		update $\leftarrow$ vertex.rank  /  |vertex.edges|\;
		\ForEach{neighbourId $\in$ vertex.neighbours}{
			Emit(neighbourId, \rank update)\;
		}
	}
	\reduce{vertexId, [p1, p2, p3, ...]}
	\Begin{
		sum $\leftarrow$ 0\;
		\ForEach{$p \in [p1, p2, p3, ...]$}{
			\eIf{p is \vertex}{
				$vertex \leftarrow p$\;
			}{
				$sum \leftarrow sum + p$\;
			}
		}
		
		vertex.pagerank $\leftarrow$ sum\;
		Emit(vertexId,  \vertex vertex)\;
	}

\end{algorithm}

==> codes/ch02_pact_cc.tex <==
\begin{algorithm}[h]
\SetKwFunction{NeighbourWithComponentJoin}{NeighbourWithComponentJoin}
\SetKwFunction{MinimumReduce}{MinimumReduce}
\Input{vertices as tuples of form (vid, vid), edges as tuples of form (source, target}
\pact{vertices, edges}
\Begin{
	\tcp{add loops to the edges set}
	edges $\leftarrow$ edges.union(vertices)\;
	
	\tcp{1) create bulk iteration on vertices}
	
	iteration $\leftarrow$ vertices.iterate(MAX\_ITERATIONS)\;
	\BlankLine
	
	
	\tcp{2) define iteration}
	updatedVertices $\leftarrow$ iteration.\;
	\Indp \Indp \Indp
	
		\BlankLine
			\tcp{join vertices with edges}
	        .join(edges).with(NeighbourWithComponentJoin)
	        
	   	\BlankLine
	        \tcp{group by vertex id and select minimum of componentId}
	        
	        .groupBy(vertexId).reduce(MinimumReduce)
	        
	\Indm \Indm \Indm
	\BlankLine
	
	\tcp{3) close iteration}
	result $\leftarrow$ iteration.closeWith(updatedVertices)\;
	
}
\tcp{user function for the join operator}
\NeighbourWithComponentJoin{vertex, edge}
\Begin{
	Emit(edge.target, vertex.componentId);
}
\MinimumReduce{vertexId, componentIds}
\Begin{
	Emit(vertexId, minimum(componentIds));
}
\caption{Connected Components in the PACT model}
\label{alg:pact_cc}
\end{algorithm}

\begin{comment}
vertices = getVertices() // tuples (vertexId, componentId), componentId = vertexId
edges = getEdges()  // tuples (sourceVertexId, targetVertexId)

// 1) create delta iteration
// initial solution and work set contain all vertices
iteration = vertices.iterateDelta(vertices, maxIterations)

// 2) define step
changedVertices = iteration.getWorkset()
        // join with the edges and 
        // create tuple (neighbourVertexId, myComponentId) for each neighbour
        .join(edges).with(new NeighbourWithComponentIDJoin())
        
        // group by vertex id and select minimum neighbour component ID
        .groupBy(0).aggregate(MIN, componentId)
        
        // update if the component ID is smaller than current one
        .join(iteration.getSolutionSet())
        .flatMap(new ComponentIdFilter())

// 3) close the iteration (set delta and new workset: both are the changed vertices)
result = iteration.closeWith(changedVertices, changedVertices)

// operator functions
class NeighbourWithComponentIDJoin
    join(vertex, edge)
        return new Tuple(edge.otherVertexId, vertex.componentId)

class ComponentIdFilter
    flatMap(vertexNew, vertexOld) 
        if (vertexNew.componentId < vertexOld.componentId)
            emit(vertexNew);
\end{comment}

==> codes/ch02_pregel_gas_emulation.tex <==
\begin{algorithm}[h]
\compute{\Vertex, \Message}
\Begin{
	\If{getSuperstep() > 0}{
		
		total = 0\tcp*[r]{Gather}
		\For{$msg \in messages$}{
			%\eIf{msg has type SIGNAL}{
			%	msg $\leftarrow$ vertex.cache[msg.sender]\;
			%}{
			%	vertex.cache[msg.sender]\ $\leftarrow$ msg\;
			%}
			total = \gathersum{total, \gather{msg}}\;
		}
		\BlankLine
		apply(\Vertex, total)\tcp*[r]{Apply}
		\BlankLine
		
		\For{$edge \in \Vertex.edges$}{
			scatter(\Vertex, edge)\tcp*[r]{Scatter}
		}
	}
	\For{$\Edge \in \Vertex.edges$}{
		\tcp{send data needed by gather to all neighbours}
		msg = relevantData(\Vertex, \Edge)\;
		sendMessage(edge.otherVertex, msg)\;
	}
}
%\signal{\Vertex}
%\Begin{
%	signalVertex[\Vertex] $\leftarrow$ true;
%}
\caption{Emulation of a GAS program in Pregel}
\label{alg:pregel_gas_emulation}
\end{algorithm}

==> codes/ch03_flink_code.tex <==
\begin{minted}[linenos=true,
               numbersep=5pt,tabsize=3,
               frame=lines,
               framesep=2mm, mathescape]{java}
public class ConnectedComponents {
	public static void main(String[] args) throws Exception {
		// set up the execution environment
		final ExecutionEnvironment env = 
				ExecutionEnvironment.getExecutionEnvironment();
		// get input data
		DataSet<Long> verticeIds = ...
		DataSet<Tuple2<Long, Long>> directedEdges = ...
		DataSet<Tuple2<Long, Long>> vertices = 
				verticeIds.map(new DuplicateMapper<Long>());
		
		// 1) create delta iteration
		DeltaIteration<Tuple2<Long, Long>, Tuple2<Long, Long>> iteration = 
				vertices.iterateDelta(vertices, MAX_ITERATIONS, 0); 
		// 2) define iteration step
		DataSet<Tuple2<Long, Long>> changedVertices = iteration.getWorkset()
			// join with edges
			.join(edges).where(0).equalTo(0).with(new NeighbourWithComponentIdJoin())
			// group by vertex id and select minimum for each vertex
			.groupBy(0).aggregate(Aggregations.MIN, 1)
			// keep in the set only if component ID is smaller than current one
			.join(iteration.getSolutionSet()).where(0).equalTo(0)
			.flatMap(new FilterSmallerIDs());	
		// 3) close iteration by setting new delta and work set
		DataSet<Tuple2<Long, Long>>result = 
				iteration.closeWith(changedVertices, changedVertices);
		
		// execute program
		env.execute("Connected Components");
	}
	public static final class DuplicateMapper<T> 
		extends MapFunction<T, Tuple2<T, T>> {
		public Tuple2<T, T> map(T value) {
			return new Tuple2<T, T>(value, value);
		}}
	public static final class NeighbourWithComponentIdJoin extends 
		JoinFunction<Tuple2<Long, Long>, Tuple2<Long, Long>, Tuple2<Long, Long>> {
		public Tuple2<Long, Long> join(Tuple2<Long, Long> vertex,
				Tuple2<Long, Long> edge) {
			Long neighbourVertexID = edge.f1;
			Long vertexComponentID = vertex.f1;
			return new Tuple2<Long, Long>(neighbourVertexID, vertexComponentID);
		}}
	public static final class FilterSmallerIDs extends FlatMapFunction
		<Tuple2<Tuple2<Long,Long>, Tuple2<Long, Long>>, Tuple2<Long, Long>> {
		public void flatMap(Tuple2<Tuple2<Long, Long>, 
			Tuple2<Long, Long>> join, Collector<Tuple2<Long, Long>> out) {
			Long newComponentID = join.f0.f1;
			Long currentComponentID = join.f1.f1;
			if(newComponentID < currentComponentID) {
				out.collect(join.f0);
			}
		}}
}
\end{minted}

==> codes/ch03_giraph++_code.tex <==
\begin{minted}[linenos=true,
               numbersep=5pt,tabsize=3,
               frame=lines,
               framesep=2mm, mathescape]{java}
public class ConnectedComponents extends AbstractSubGraph<LongWritable, 
			LongWritable, NullWritable, LongWritable> {
	@Override
	public void compute(
			Partition<LongWritable, LongWritable, NullWritable, LongWritable> subgraph)
			throws IOException {
		if(getSuperstep()==0) {
			// sequentialConnectedComponents(subgraph);
			
		} else {
			updateLabelMapping(subgraph);
			updateVertexLabels(subgraph);
		}
			
	}
}
\end{minted}

==> codes/ch03_giraph_code.tex <==
\begin{minted}[linenos=true,
               numbersep=5pt,tabsize=3,
               frame=lines,
               framesep=2mm, mathescape]{java}
public class ConnectedComponents extends
	BasicComputation<IntWritable, IntWritable, NullWritable, IntWritable> {

	public void compute(Vertex<IntWritable, IntWritable, NullWritable> vertex,
			Iterable<IntWritable> messages) {
		boolean changed = false;
		if (getSuperstep() == 0) {
			vertex.setValue(vertex.getId());  // initalize label with vertex id
			changed = true;
		} else {
			// new lower component label?
			for (IntWritable neighbourComponentId : messages) {
				if (neighbourComponentId.get() < vertex.getValue().get()) {
					changed = true;
					vertex.setValue(neighbourComponentId);
				}
			}
		}
		if (changed) {		// send new label to neighbours
			sendMessageToAllEdges(vertex, vertex.getValue());
		}
		vertex.voteToHalt();
	}
}
\end{minted}

==> codes/ch03_giraph_mastercompute.tex <==
\begin{minted}[linenos=true,
               numbersep=5pt,tabsize=3,
               frame=lines,
               framesep=2mm, mathescape]{java}
public static final class MyMasterCompute extends DefaultMasterCompute {	
	@Override
	public void initialize() {
		registerAggregator(CONVERGED, BooleanAndAggregator.class);
	}			
	@Override
	public void compute() {
			boolean converged = 
				this.<BooleanWritable>getAggregatedValue(CONVERGED).get();
			if(converged) {
				haltComputation();
			}
	}
}
\end{minted}

==> codes/ch03_graphlab_code.tex <==
\begin{minted}[linenos=true,
               numbersep=5pt,
               frame=lines,texcl=true,
               framesep=2mm, mathescape]{c++}
#include <graphlab.hpp>
typedef graphlab::distributed_graph<double, graphlab::empty> graph_type; //$\label{line:ch03_grlc_declaration}$
struct min_gather {    // minimum gather type with customized sum operator
    int min;
    min_gather(v) : min(v) {}
    min_gather& operator+=(const min_gather& other) { //$\label{line:ch03_grlc_sum}$
        if (min > other.min) min = other.min;
        return (*this);
    }
};
class cc_program :      // Connected Components vertex program
public graphlab::ivertex_program<graph_type, min_gather>, //$\label{line:ch03_grlc_declarationg}$
public graphlab::IS_POD_TYPE {
public:
    bool changed;
    edge_dir_type gather_edges(icontext_type& c, const vertex_type& v) const {
        return graphlab::ALL_EDGES; // gather on ALL edges $\label{line:ch03_grlc_gather_edges}$
    }
    min_gather gather(icontext_type& context, 
    		const vertex_type& vertex, edge_type& edge) const {
        vertex_type otherVertex = (edge.source().id() == vertex.id()) 
        				? edge.target() : edge.source();  
        return min_gather(otherVertex.data()); // gather neighbour's component id
    }
    void apply(icontext_type& context, vertex_type& vertex, const gather_type& min) {
        this->changed = false;
        if (min.min < vertex.data().component_id) {     
            this->changed = true;   // found lower component id
            vertex.data().component_id = min.min;
        }
    }
    edge_dir_type scatter_edges(icontext_type& c, const vertex_type& v) const {
        if (this->changed)return graphlab::ALL_EDGES;  // signal only if component  $\label{line:ch03_grlc_scatter_edges}$
        else return graphlab::NO_EDGES;                // id has changed
    }
    void scatter(icontext_type& c,
            const vertex_type& vertex, edge_type& edge) const {
        vertex_type otherVertex = (edge.source().id() == vertex.id()) 
        				? edge.target() : edge.source();
        context.signal(otherVertex);
    }
};
int main(int argc, char** argv) {
    graph.load("graph_file" , line_parser);    // load graph from file $\label{line:ch03_grlc_parser}$
    graphlab::mpi_tools::finalize();           // with a line\_parser function
    graphlab::omni_engine<cc_program> engine(dc, graph, "sync"); // $\label{line:ch03_grlc_engine}$
    engine.signal_all();
    engine.start();   // start vertex program in synchronous engine
    graph.save("output", graph_writer(), false, true, false);   // output graph $\label{line:ch03_grlc_output}$
}
\end{minted}

==> codes/ch04_cc_giraph++.tex <==
\begin{algorithm}[h]
\compute{vertex, messages}
\Begin{
}
\combine{msg1, msg2}
\Begin{
	\KwRet{min(msg1, msg2)}
}
\caption[Connected Components in Pregel]{CC in Pregel}
\label{alg:pregel_cc}
\end{algorithm}

==> codes/ch04_cc_pregel.tex <==
\begin{algorithm}[h]
\compute{vertex, messages}
\Begin{
	\eIf{getSuperstep() = 0}{
		\tcc{optimized first superstep: choose minimum directly }
		vertex.component $\leftarrow$ minimum(vertex.edges)\;
		\If{vertex.component $\neq$ vertex.id}{
			\ForEach{neighbourId in vertex.neighbourIds} {
				\If{neighbourId > vertex.component} {
					\sendmsg{neigbourId, vertex.component}
				}
			}
		}
	}{
		minMsg $\leftarrow$ getMinumum(messages)\;
		\If{msg < vertex.component}{
			\tcp{found smaller component}
			vertex.component $\leftarrow$ msg\;

			sendToAll(msg)\;
		}
	}
	vertex.voteToHalt()\;
}
\combine{msg1, msg2}
\Begin{
	\KwRet{min(msg1, msg2)}
}
\caption[Connected Components in Pregel]{CC in Pregel}
\label{alg:pregel_cc}
\end{algorithm}

==> codes/ch04_cdlabel_gas.tex <==
\begin{algorithm}[b]
%\init{vertex}
%\Begin{
%	vertex.rank $\leftarrow$ 1\;
%}
\tcp{gather on incoming edges}
\gather{vertex, edge}
\Begin{
	frequencyMap $\leftarrow$ new Map\;
	frequencyMap.put((edge.source.label, 1))\;
	\KwRet{frequencyMap}
}
\gathersum{map1, map2}
\Begin{
	\ForEach{(label, freq) $\in$ map2}{
		map1.put(label, freq + map1.get(label)) \tcp*[r]{combine two maps}
	}
	\KwRet{map1}
}
\apply{vertex, frequencyMap}
\Begin{
	mostFrequent $\leftarrow$ frequencyMap.getMostFrequentEntries\;
	newLabel $\leftarrow$ chooseRandom(mostFrequent)\;
	\eIf{newLabel $\neq$ vertex.label}{
		vertex.label $\leftarrow$ newLabel\;
		converged $\leftarrow$ FALSE\;
	}{
		converged $\leftarrow$ TRUE\;
	}
}
\tcp{scatter on outgoing edges}
\scatter{vertex, edge}
\Begin{
	\If{changed}{
		\signal{edge.target}
	}
}
\caption{Community Detection using Label Propagation in GAS}
\label{alg:cdlabel_gas}
\end{algorithm}
\begin{comment}

    // for each in-edge gather the label
    most_frequent_gather gather(icontext_type& context, const vertex_type& vertex,
            edge_type& edge) const {
        most_frequent_gather label;
        
        label.occurrences.insert(unordered_map::value_type(edge.source().data(), 1));
        return label;
    }

    // gather result contains the label map with the occurrences of neigbour labels
    void apply(icontext_type& context, vertex_type& vertex,
            const gather_type& labelmap) {
        vertex_data_type newlabel = get_most_frequent(labelmap.occurrences);
        
        if(newlabel != -1) {
            if(vertex.data() == newlabel) {
                converged = true;
            } else {
                converged = false;
                vertex.data() = newlabel;
            }
        }
        //context.cout() << context.iteration() << ") vertex " << vertex.id() << " new label: " << newlabel << "\n";
        //context.signal(vertex);
    }

    // returns the most frequent label in the given map. if the map is empty, -1 is returned.
    vertex_data_type get_most_frequent(unordered_map occurrences) {
        vertex_data_type most_frequent_label = -1;
        int most_frequent_label_occurrences = -1;
        
        for(unordered_map::const_iterator it = occurrences.begin(); it != occurrences.end(); ++it) {
            if(it->second > most_frequent_label_occurrences
                    || (it->second == most_frequent_label_occurrences && it->first < most_frequent_label)) {
                
                most_frequent_label = it->first;
                most_frequent_label_occurrences = it->second;
            }
        }
        return most_frequent_label;
    }

    // DONT SCATTER
    edge_dir_type scatter_edges(icontext_type& context,
            const vertex_type& vertex) const {
        if(converged) {
            return graphlab::NO_EDGES;
        } else {
            return graphlab::OUT_EDGES;
        }
    }
    
    void scatter(icontext_type& context, const vertex_type& vertex, edge_type& edge) const {
        context.signal(edge.target());
    }
};

\end{comment}

==> codes/ch04_cdlabel_giraph++.tex <==
\begin{algorithm}[b]
\compute{vertex, messages}
\Begin{
	\ForEach{vertex $\in$ internalVertices}{
		\If{getAggregatorValue(CONVERGENCE)}{
			vertex.voteToHalt()\tcp*[r]{algorithm converged}
		}
		\eIf{getSuperstep() = 0}{
			\eIf{vertex.degree > 0}{
				\tcp{no need to initialize label with id - vertex knows neighbours' ids}
				vertex.label $\leftarrow$ chooseRandom(vertex.neighbourIds)\;
			}{
				vertex.label $\leftarrow$ vertex.id\;
				vertex.voteToHalt()\;
			}
		}{
			mostFrequent $\leftarrow$ getMostFrequentValues(vertex.messages $\cup$ vertex.internalNeighbourLabels)\;
			newLabel $\leftarrow$ chooseRandom(mostFrequent)\;
			\eIf{newLabel $\neq$ vertex.label}{
				vertex.label $\leftarrow$ newLabel\;
				converged $\leftarrow$ FALSE\;
			}{
				converged $\leftarrow$ TRUE\;
			}
			setAggregatorValue(CONVERGENCE, converged)\;
		}
	}
}
\caption{Community Detection using Label Propagation in Giraph++}
\label{alg:cdlabel_giraph++}
\end{algorithm}

==> codes/ch04_cdlabel_pact.tex <==
\begin{algorithm}[h]
\SetKwFunction{randomselect}{InitialSelectReducer}
\SetKwFunction{neighbourjoin}{NeighbourWithLabelJoin}
\SetKwFunction{labelSelector}{LabelSelector}
\SetKwFunction{filterChanged}{changedFilter}
\Input{vertices as tuples of form (vid, vid), edges as tuples of form (vid1, vid2)}
\pact{vertices, edges}
\Begin{
	\tcp{First iteration: Choose random neighbour as label}
	firstIteration $\leftarrow$ edges.project(1,0).group(0).reduce(\randomselect)\;

	\tcp{1) create bulk iteration on vertices}
		
	iteration $\leftarrow$ firstIteration.iterate(MAX\_ITERATIONS)\;
	\BlankLine
	
		
	\tcp{2) define iteration}
	updatedVertices $\leftarrow$ iteration.\;
	\Indp \Indp \Indp
	
		\BlankLine
			\tcp{join vertices with edges and create tuple (neighbourVertexID, myLabel) for each neighbour}
      		.join(edges).with(\neighbourjoin)
     
	   	\BlankLine
			\tcp{group by vertex id and label aggregate count: creates set with tuples (vertex, label, count)}
			.groupBy(vertexId, label).aggregateSum()

	   	\BlankLine
			\tcp{select most frequent}
			.groupBy(vertexId).reduce(\labelSelector)\;
		
			
	      
	\Indm \Indm \Indm
	\BlankLine

	changedVertices $\leftarrow$ updatedVertices.\;
	\Indp \Indp \Indp
							
	   	\BlankLine
			\tcp{only keep vertices with changed label}
			.join(iteration).with(\filterChanged)\;			
			
	      
	\Indm \Indm \Indm
	\BlankLine	
	\tcp{3) close iteration \\ with new work set and delta set}
	result $\leftarrow$ iteration.closeWith(updatedVertices, changedVertices)\;
	
	
}
\randomselect{vertexId, labelIds}
\Begin{
	\emit{(vertexId, getRandom(labelIds))}
}
\neighbourjoin{vertex, edge}
\Begin{
	\emit{(edge.target, vertex.label)}
}
\labelSelector{vertexId, labels}
\Begin{
	mostFrequentLabels = getMostFrequent(labels)\;
	selectedLabel = getRandom(mostFrequentLabels)\;
	\emit{(vertexId, selectedLabel)}
}
\filterChanged{oldVertex, newVertex}
\Begin{
	\If{oldVertex.label $\neq$ newVertex.label}{
		\emit{newVertex}
	}
}
\caption{Community Detection in the PACT model}
\label{alg:cdlabel_pact}
\end{algorithm}
\begin{comment}

		// get vertices and initialize value with vertex id
		DataSet<Tuple2<Long, Long>> vertices = edges.groupBy(0).reduce(new ReduceFunction<Tuple2<Long, Long>>() {

			@Override
			public Tuple2<Long, Long> reduce(Tuple2<Long, Long> value1,
					Tuple2<Long, Long> value2) throws Exception {
				return new Tuple2<Long, Long>(value1.f0, value1.f0);
			}
			
		});

		// 1) create delta iteration
		// initial solution and work set contain all vertices
		IterativeDataSet<Tuple2<Long, Long>> iteration = vertices.iterate(MAXITERATIONS); 
		

		// 2) define iteration step
	
		DataSet<Tuple2<Long, Long>> verticesWithNewLabel = iteration
				
				// join with edges and
				// create tuple (neighbourVertexID, myLabelId) for each neighbour
				.join(edges).where(0).equalTo(0).with(new NeighbourWithLabelJoin())
				
				// group by vertex id
				.groupBy(0, 1).reduceGroup(new LabelReducer())
				.groupBy(0).reduceGroup(new MostFrequentLabelReducer());

		DataSet<Long> changedVertices = verticesWithNewLabel.join(vertices).where(0).equalTo(0).flatMap(new KeepChangedLabelsMap());
		// 3) close iteration

		DataSet<Tuple2<Long, Long>> result = iteration.closeWith(verticesWithNewLabel, changedVertices);
		//result.print();
	
\end{comment}

==> codes/ch04_cdlabel_pregel.tex <==
\begin{algorithm}[b]
\compute{vertex, messages}
\Begin{
	\eIf{getSuperstep() = 0}{
		\eIf{vertex.degree > 0}{
			\tcp{no need to initialize label with id - vertex knows neighbours' ids}
			vertex.label $\leftarrow$ chooseRandom(vertex.neighbourIds)\;
		}{
			vertex.label $\leftarrow$ vertex.id\;
			voteToHalt()\;
		}
	}{
		\eIf{getAggregatorValue(CONVERGENCE)}{
			voteToHalt()\tcp*[r]{algorithm converged}
		}{
			mostFrequent $\leftarrow$ getMostFrequentMessage(messages)\;
			newLabel $\leftarrow$ chooseRandom(mostFrequent)\;
			\eIf{newLabel $\neq$ vertex.label}{
				vertex.label $\leftarrow$ newLabel\;
				converged $\leftarrow$ FALSE\;
			}{
				converged $\leftarrow$ TRUE\;
			}
			setAggregatorValue(CONVERGENCE, converged)\;
			sendMessageToAllBoundaryEdges(\vertex, \vertex.label)\;
		}
	}
}
\caption{Community Detection using Label Propagation in Pregel}
\label{alg:cdlabel_pregel}
\end{algorithm}


==> codes/ch04_clustering_giraph++.tex <==
\begin{algorithm}[h]
\SetKwData{Newrank}{newrank}
\compute{vertex, messages}
\Begin{
	\ForEach{v $\in$ internalVertices}{
	
		\If{getSuperstep() = 0}{
			\ForEach{bn $\in$ v.boundaryNeighbours}{
				\ForEach{m $\in$ v.neighbours}{
					sendMessage(bn, m.id)\;
				}
			}
		}
		\ElseIf{getSuperstep() = 1}{
			neighbourEdges $\leftarrow$ 0\;
			\ForEach{msg $\in$ vertex.messages} {
				\If{msg $\in$ vertex.neighbours}{
					neighbourEdges $\leftarrow$ neighbourEdges + 1\;
				}
			}
			\ForEach{in $\in$ vertex.internalNeighbours}{
				commonNeighbours $\leftarrow$ intersection(v.neighbours, in.neighbours)\;
				neighbourEdges $\leftarrow$ neighbourEdges + commonNeighbours.size()\;
			}
			
			neighbourEdges $\leftarrow$ neighbourEdges / 2 \tcp*[r]{each link has a message from both vertices}
			possibleEdges $\leftarrow$ vertex.numEdges * (vertex.numEdges - 1) / 2\;
			vertex.localClustering $\leftarrow$ neighbourEdges / possibleEdges\;
			
			\tcp{Use aggregators for global values, like in Pregel}
		}
	}
}
\caption{Clustering Coefficients in Giraph++}
\label{alg:clustering_giraph++}
\end{algorithm}

==> codes/ch04_clustering_pact.tex <==
\begin{algorithm}[h]
\SetKwFunction{CommonNeighbourMapper}{CommonNeighbourMapper}
\SetKwFunction{LocalCCMapper}{LocalCCMapper}
\SetKwFunction{PossibleLinksReducer}{PossibleLinksReducer}
\SetKwFunction{SumReducer}{SumReducer}
\Input{vertices as tuples of form (vid, 1), edges as tuples of form (vid1, vid2)}
\pact{vertices, neighbours}
\Begin{

	neighbourNeighbours $\leftarrow$ edges.join(edges).project(0,1,3)\;
	commonNeighbours $\leftarrow$ neighboursNeighbours.join(edges).where(0).equalTo(0)\;	
		\Indp \Indp \Indp
		.flatMap(\CommonNeighbourMapper)\;
		\Indm \Indm \Indm
	
	linksPerVertex $\leftarrow$ commonNeighbours.group(0).aggregate(SUM)\;
	
	possibleLinksPerVertex $\leftarrow$ edges.group(0).reduce(\PossibleLinksReducer)\;
	\BlankLine
	localCCs $\leftarrow$ linksPerVertex.join(possibleLinksPerVertex).flatMap(\LocalCCMapper)\;
	
	totalLinks $\leftarrow$ linksPerVertex.project(1).reduce(SumReducer)\;
	totalPossibleLinks $\leftarrow$ possibleLinksPerVertex.project(1).reduce(SumReducer)\;
	totalLocalCC $\leftarrow$ localCCs.project(1).reduce(SumReducer)\;
	\BlankLine
	globalCC $\leftarrow$ totalLinks / totalPossibleLinks\;
	localAvgCC $\leftarrow$ totalLocalCC / numVertices\;
	
	
}
\CommonNeighbourMapper{vertex, neighbourA, neighbourAneighbour, neighbourB}
\Begin{
	\If{neighbourAneighbour = neighbourB}{
		\emit{(vertex, 1)}
	}
}
\PossibleLinksReducer{vertex, neighbourList}
\Begin{
	possibleLinks $\leftarrow$ neighbourList.size * (neighbourList.size - 1) / 2\;
	\emit{vertex, possibleLinks}
}
\LocalCCMapper{vertexA, vertexB}
\Begin{
	cc $\leftarrow$ vertexA.links / vertexB.possibleLinks\;
	
	
	\emit{(vertexA.id, cc)}
}
\SumReducer{a, b} 
\Begin{
	\KwRet{a + b}
}
\caption{Clustering Coefficients in the PACT model}
\label{alg:clustering_pact}
\end{algorithm}
\begin{comment}

DataSet<Tuple3<Long, Long, Long>> neighboursNeighbours = edges.join(edges).where(1).equalTo(0)
		.projectFirst(0,1).projectSecond(1).types(Long.class,  Long.class,  Long.class);
//neighboursNeighbours.print();

DataSet<Tuple2<Long, Long>> commonNeighbours = neighboursNeighbours.join(edges).where(0).equalTo(0).flatMap(new CommonNeighbourMapper());
//commonNeighbours.print();


DataSet<Tuple2<Long, Long>> triangles = commonNeighbours.groupBy(0).aggregate(Aggregations.SUM, 1);
//triangles.print();

DataSet<Tuple2<Long, Long>> numberOfNeighbours = edges.map(new OneMapper())
		.groupBy(0).aggregate(Aggregations.SUM, 1);
//numberOfNeighbours.print();


// Local ClusteringCoefficient
DataSet<Tuple2<Long, Double>> clusteringCoefficients = triangles
		.join(numberOfNeighbours).where(0).equalTo(0).with(new CalculateClusteringCoefficient());
		
//clusteringCoefficients.print();

// Local average

DataSet<Tuple1<Double>> localSum = clusteringCoefficients
		.aggregate(Aggregations.SUM, 1).project(1).types(Double.class);
DataSet<Tuple1<Long>> numberOfVertices = vertices.map(new VertexOneMapper<Tuple1<Long>>()).aggregate(Aggregations.SUM, 0);
DataSet<Double> lccAvg = localSum
		.cross(numberOfVertices).with(new DivideCross());

lccAvg.print();

// Global Clustering Coefficient

// sum of all triangles
DataSet<Tuple1<Long>> triangleSum = triangles
		.aggregate(Aggregations.SUM, 1).project(1).types(Long.class);

// sum of all possible triangles
DataSet<Tuple1<Long>> possibleTriangleSum = numberOfNeighbours
		.map(new PossibleTrianglesMapper()).aggregate(Aggregations.SUM, 0);

DataSet<Double> gcc = triangleSum
		.cross(possibleTriangleSum).with(new  CalculateGlobalClusteringCoefficient());
	
	
\end{comment}

==> codes/ch04_pagerank_giraph++.tex <==
\begin{algorithm}[h]
\SetKwData{Newrank}{newrank}
\compute{vertex, messages}
\Begin{
	\ForEach{v $\in$ internalVertices}{
		sum $\leftarrow$ sum(v.messages)\;
		\ForEach{ n $\in$ v.internalNeighbours}{
			sum $\leftarrow$ sum + n.rank\;
		}
		v.rank $\leftarrow$ $\alpha$ + (1 - $\alpha$) * sum\;
		
		msg $\leftarrow$ v.rank / v.numEdges\;
		\ForEach{ n $\in$ v.boundaryNeighbours}{
			sendMessage(n, msg)\;
		}
	}
}
\combine{msg1, msg2}
\Begin{
	\KwRet{msg1 + msg2}
}
\caption{PageRank in Giraph++}
\label{alg:pagerank_giraph++}
\end{algorithm}

==> codes/ch04_pagerank_giraph++_accumulative.tex <==
\begin{algorithm}[b]
\SetKwData{Newrank}{newrank}
\compute{vertex, messages}
\Begin{
	\eIf{getSuperstep() > MAX\_ITERATION}{
		allVoteToHalt();
	}{
		\If{getSuperstep() = 0}{
			\ForEach{v $\in$ allVertices}{
				v.rank $\leftarrow$ 0\;
				v.delta $\leftarrow$ 0\;
			}
		}
		\ForEach{iv $\in$ activeInternalVertices}{
			\If{getSuperstep() = 0}{
				iv.delta $\leftarrow$ iv.delta +  $\alpha$\;
			}
			iv.delta $\leftarrow$ iv.delta + sum(iv.messages)\;
			\If{iv.delta > 0}{
				iv.rank $\leftarrow$ iv.rank + iv.delta\;
				update $\leftarrow$ (1 - $\alpha$) * iv.delta / iv.numEdges\;
				
				\ForEach{neighbour $\in$ iv.neighbours}{
					neighbour.delta $\leftarrow$ neighbour.delta + update
				}
			}
			iv.delta $\leftarrow$ 0\;
		}
		\ForEach{bv $\in$ boundaryVertices}{
			\If{bv.delta > 0}{
				sendMsg(bv, bv.delta)\;
				bv.delta $\leftarrow$ 0\;
			}
		}
	}
}
\combine{msg1, msg2}
\Begin{
	\KwRet{msg1 + msg2}
}
\caption[PageRank in Giraph++, Accumulative Iterative Update algorithm]{Accumulative Iterative Update algorithm of PageRank in Giraph++ \cite{giraph++}}
\label{alg:pagerank_giraph++_accumulative}
\end{algorithm}

==> codes/ch04_pagerank_pact.tex <==
\begin{algorithm}[h]
\SetKwFunction{PageRankMap}{PageRankMap}
\SetKwFunction{Dampener}{Dampener}
\SetKwFunction{NotConvergedFilter}{NotConvergedFilter}
\Input{vertices as tuples of form (vid, 1), neighbour list as tuples of form (vid, [neighbour\_id1, neighbour\_id2])}
\pact{vertices, neighbours}
\Begin{
	\tcp{1) create bulk iteration on vertices}
	
	iteration $\leftarrow$ vertices.iterate(MAX\_ITERATIONS)\;
	\BlankLine
	
	\tcp{2) define iteration}
	newRanks $\leftarrow$ iteration.\;
	\Indp \Indp \Indp
	
		\BlankLine
			\tcp{join with neighbours and apply pagerank function}
			.join(neighbours).where(0).equalTo(0).flatMap(\PageRankMap)
      
	   	\BlankLine
	      	\tcp{group by vertex id and aggregate sum of all ranks}
	     	.groupBy(0).aggregate(SUM, 1)
	      
		\BlankLine
			\tcp{add dampening factor}
			.map(\Dampener)\;
      
	\Indm \Indm \Indm
	\BlankLine
	
	notConvergedVertices $\leftarrow$ iteration.\;
	\Indp \Indp \Indp
		
		\BlankLine
			\tcp{filter converged vertices}
			.join(newRanks).where(0).equalTo(0).flatMap(\NotConvergedFilter)\;
	
	\Indm \Indm \Indm
	\BlankLine
		
	\tcp{3) close iteration}
	result $\leftarrow$ iteration.closeWith(newRanks, notConvergedVertices)\;
}
\PageRankMap{vertex, neighbours}
\Begin{
	rank $\leftarrow$ vertex.rank / neighbours.list.length\;
	\ForEach{n $\in$ neighbours.list}{
		\emit{Tuple(n.id, rank)}
	}
}
\Dampener{vertex}
\Begin{
	\vertex.rank $\leftarrow$ $\alpha$ + (1 - $\alpha$) * \vertex.rank\;
	\KwRet{\vertex}
%($\alpha$, numVertices)
}
\NotConvergedFilter{oldVertex, newVertex}
\Begin{
	delta $\leftarrow$ |newVertex.rank - oldVertex.rank|\;
	\If{delta > TOLERANCE}{
		\emit{newVertex}
	}
}
\caption{PageRank in the PACT model}
\label{alg:pagerank_pact}
\end{algorithm}


==> codes/ch04_pagerank_pregel_accumulative.tex <==
\begin{algorithm}[t]
\SetKwData{Newrank}{newrank}
\compute{vertex, messages}
\Begin{
	\If{getSuperstep() < MAX\_ITERATION}{
		delta $\leftarrow$ 0\;
	
		\If{getSuperstep() = 0}{
			delta $\leftarrow$ $\alpha$\;
			\vertex.\Rank $\leftarrow$ 0\;
		}
		delta $\leftarrow$ sum(messages);
		
		\If{ delta > 0}{
			\vertex.\Rank $\leftarrow$ \vertex.\Rank + delta\;
			sendMessageToAllEdges((1 - $\alpha$) * delta / \vertex.numEdges)\;
		}
		voteToHalt()\;
	}
}
\caption[PageRank in Pregel, Accumulative Iterative Update algorithm]{Accumulative Iterative Update algorithm of PageRank in Pregel \cite{giraph++}}
\label{alg:pagerank_pregel_accumulative}
\end{algorithm}

==> codes/ch04_sssp_gas.tex <==
\begin{algorithm}[h]
\tcp{gather on incoming edges}
\gather{vertex, edge}
\Begin{
	\KwRet{edge.sourceVertex.distance + edge.weight}
}
\gathersum{val1, val2}
\Begin{
	\KwRet{min(val1, val2)}
}
\apply{vertex, min}
\Begin{
	\If{min < vertex.distance}{
		changed $\leftarrow$ true\;
		vertex.distance = min\;
	}
}
\tcp{scatter on outgoing edges}
\scatter{vertex, edge}
\Begin{
	\If{changed}{
		\signal{edge.targetVertex}
	}
}
\caption{SSSP in GAS}
\label{alg:gas_sssp}
\end{algorithm}

\begin{comment}
class label_propagation: public graphlab::ivertex_program<graph_type, size_t,
    min_message>, public graphlab::IS_POD_TYPE {
private:
  size_t recieved_labelid;
  bool perform_scatter;
public:
  label_propagation() {
    recieved_labelid = std::numeric_limits<size_t>::max();
    perform_scatter = false;
  }

  //receive messages
  void init(icontext_type& context, const vertex_type& vertex,
      const message_type& msg) {
    recieved_labelid = msg.value;
  }

  //do not gather
  edge_dir_type gather_edges(icontext_type& context,
      const vertex_type& vertex) const {
    return graphlab::NO_EDGES;
  }
  size_t gather(icontext_type& context, const vertex_type& vertex,
      edge_type& edge) const {
    return 0;
  }

  //update label id. If updated, scatter messages
  void apply(icontext_type& context, vertex_type& vertex,
      const gather_type& total) {
    if (recieved_labelid == std::numeric_limits<size_t>::max()) {
      perform_scatter = true;
    } else if (vertex.data().labelid > recieved_labelid) {
      perform_scatter = true;
      vertex.data().labelid = recieved_labelid;
    }
  }

  edge_dir_type scatter_edges(icontext_type& context,
      const vertex_type& vertex) const {
    if (perform_scatter)
      return graphlab::ALL_EDGES;
    else
      return graphlab::NO_EDGES;
  }

  //If a neighbor vertex has a bigger label id, send a massage
  void scatter(icontext_type& context, const vertex_type& vertex,
      edge_type& edge) const {
    if (edge.source().id() != vertex.id()
        && edge.source().data().labelid > vertex.data().labelid) {
      context.signal(edge.source(), min_message(vertex.data().labelid));
    }
    if (edge.target().id() != vertex.id()
        && edge.target().data().labelid > vertex.data().labelid) {
      context.signal(edge.target(), min_message(vertex.data().labelid));
    }
  }
};
\end{comment}

==> codes/ch04_sssp_gas_messagebased.tex <==
\begin{algorithm}[h]
\messagesum{m1, m2}
\Begin{
	\KwRet{min(val1, val2)}
}
\apply{vertex, msg}
\Begin{
	\If{msg < vertex.distance}{
		changed $\leftarrow$ true\;
		vertex.distance = msg\;
	}
}
\tcp{scatter on outgoing edges}
\scatter{vertex, edge}
\Begin{
	\If{changed $\land$ edge.targetVertex.distance > vertex.distance}{
		msg $\leftarrow$ vertex.distance + edge.weight\;
		\sendmsg{edge.targetVertex, msg}
	}
}
\caption[SSSP in GraphLab]{SSSP in GraphLab using the GraphLab message library}
\label{alg:sssp_gas_message}
\end{algorithm}

\begin{comment}
class label_propagation: public graphlab::ivertex_program<graph_type, size_t,
    min_message>, public graphlab::IS_POD_TYPE {
private:
  size_t recieved_labelid;
  bool perform_scatter;
public:
  label_propagation() {
    recieved_labelid = std::numeric_limits<size_t>::max();
    perform_scatter = false;
  }

  //receive messages
  void init(icontext_type& context, const vertex_type& vertex,
      const message_type& msg) {
    recieved_labelid = msg.value;
  }

  //do not gather
  edge_dir_type gather_edges(icontext_type& context,
      const vertex_type& vertex) const {
    return graphlab::NO_EDGES;
  }
  size_t gather(icontext_type& context, const vertex_type& vertex,
      edge_type& edge) const {
    return 0;
  }

  //update label id. If updated, scatter messages
  void apply(icontext_type& context, vertex_type& vertex,
      const gather_type& total) {
    if (recieved_labelid == std::numeric_limits<size_t>::max()) {
      perform_scatter = true;
    } else if (vertex.data().labelid > recieved_labelid) {
      perform_scatter = true;
      vertex.data().labelid = recieved_labelid;
    }
  }

  edge_dir_type scatter_edges(icontext_type& context,
      const vertex_type& vertex) const {
    if (perform_scatter)
      return graphlab::ALL_EDGES;
    else
      return graphlab::NO_EDGES;
  }

  //If a neighbor vertex has a bigger label id, send a massage
  void scatter(icontext_type& context, const vertex_type& vertex,
      edge_type& edge) const {
    if (edge.source().id() != vertex.id()
        && edge.source().data().labelid > vertex.data().labelid) {
      context.signal(edge.source(), min_message(vertex.data().labelid));
    }
    if (edge.target().id() != vertex.id()
        && edge.target().data().labelid > vertex.data().labelid) {
      context.signal(edge.target(), min_message(vertex.data().labelid));
    }
  }
};
\end{comment}

==> codes/ch04_sssp_giraph++.tex <==
\begin{algorithm}[h]
\SetKwFunction{propagatechange}{propagateChange}
\compute{vertex, messages}
\Begin{
	changed $\leftarrow$ false\;
	\eIf{getSuperstep() = 0}{
		\tcc{first superstep: initialize values }
		\ForEach{v $\in$ internalVertices}{
			\eIf{v.id = source}{
				v.distance $\leftarrow$ 0\;
			}{
				v.distance $\leftarrow$ $\infty$\;
			}
		}
		\propagatechange{source, 0}
	}{
		\ForEach{v $\in$ internalVertices}{
			minMsg $\leftarrow$ getMinumum(messages)\;
			\If{minMsg < vertex.distance}{
				\tcp{found smaller distance}
				vertex.distance $\leftarrow$ minMsg\;
				\propagatechange{source, minMsg}
			}
		}
	}
}
\propagatechange{vertex, newDistance}
\Begin{
	\ForEach{e $\in$ vertex.edges}{
		neighbour $\leftarrow$ e.targetVertex\;
		\eIf{neighbour is internal}{
			\If{neighbour.distance > (newDistance + e.weight)}{
				neighbour.distance $\leftarrow$ newDistance + e.weight\;
				\propagatechange{neighbour, neighbour.distance}
			}
		}{
			msg $\leftarrow$ newDistance + e.weight\;
			sendMsg(neighbour, msg)\;
		}
	}
}
\combine{msg1, msg2}
\Begin{
	\KwRet{min(msg1, msg2)}
}
\caption{SSSP in Giraph++}
\label{alg:sssp_girpah++}
\end{algorithm}

\begin{comment}
\end{comment}

==> codes/ch04_sssp_pact.tex <==
\begin{algorithm}[h]
\SetKwFunction{initdistance}{initDistance}
\SetKwFunction{njoin}{NeighbourWithNewDistanceJoin}
\SetKwFunction{MinimumReduce}{MinimumReduce}
\SetKwFunction{filterdistance}{FilterDistance}
\Input{vertex ids , edges as tuples of form (vid1, vid2, weight)}
\pact{vertices, edges}
\Begin{

	vertices $\leftarrow$ vertexIds.map(\initdistance);
	
	initialWorkSet $\leftarrow$ (source, 0)\;
	
	\tcp{1) create delta iteration on vertices}
		
	iteration $\leftarrow$ vertices.iterateDelta(initialWorkSet, MAX\_ITERATIONS)\;
	\BlankLine
	
		
	\tcp{2) define iteration}
	changedVertices $\leftarrow$ iteration.getWorkSet()\;
	\Indp \Indp \Indp
	
		\BlankLine
			\tcp{join vertices with edges and create tuple (neighbourVertexID, vertex.distance + edge.weight) for each neighbour}
      		.join(edges).with(\njoin)
     
	   	\BlankLine
			\tcp{group by vertex id and select minimum of componentId}
			.groupBy(vertexId).reduce(MinimumReduce)
			
			// keep in the set only if component ID is smaller than current one
						
							
	   	\BlankLine
			\tcp{only keep vertices with distances lower than current one}
			.join(iteration.getSolutionSet()).with(\filterdistance)\;			
			
	      
	\Indm \Indm \Indm
	\BlankLine
	
	\tcp{3) close iteration \\ both work set and delta set are the changed vertices}
	result $\leftarrow$ iteration.closeWith(changedVertices, changedVertices)\;
}
\initdistance{vertexId}
\Begin{
	\eIf{vertexId = source}{
		\emit{(vertexId, 0)}
	}{
		\emit{(vertexId, $\infty$)}
	}
}
\njoin{vertex, edge}
\Begin{
	\KwRet{(vertex.id, vertex.distance + edge.weight)}
}

\MinimumReduce{vertexId, distances}
\Begin{
	Emit(vertexId, minimum(distances))\;
}
\filterdistance{vertexCurrent, vertexNew}
\Begin{
	\If{vertexNew.distance < vertexCurrent.distance}{
		Emit(vertexNew)\;
	}
}
\caption{SSSP in the PACT model}
\label{alg:sssp_pact}
\end{algorithm}

\begin{comment}

		
		DataSet<Tuple2<Long, Double>> vertices = verticeIds.map(new InitializeDistances(sourceVertexID));
		DataSet<Tuple2<Long, Double>> initalWorkSet = vertices.filter(new FilterSourceVertex(sourceVertexID));

		// 1) create delta iteration
		// initial solution and work set contain all vertices
		// Keypositions?
		DeltaIteration<Tuple2<Long, Double>, Tuple2<Long, Double>> iteration = vertices.iterateDelta(initalWorkSet, 30, 0); 
		
		// 2) define iteration step
		DataSet<Tuple2<Long, Double>> changedVertices = iteration.getWorkset()
				
				// join with edges and
				// create tuple (neighbourVertexID, vertex.distance + edge.weight) for each neighbour
				.join(edges).where(0).equalTo(0).with(new NeighbourWithNewDistanceJoin())
				
				// group by vertex id and select minimum for each vertex
				.groupBy(0).aggregate(Aggregations.MIN, 1)
				
				// keep in the set only if component ID is smaller than current one
				.join(iteration.getSolutionSet()).where(0).equalTo(0).flatMap(new FilterSmallerDistance())
				
				;
		// 3) close iteration by setting new delta and work set
		//    (both are the changed vertices)
		DataSet<Tuple2<Long, Double>>result = iteration.closeWith(changedVertices, changedVertices);
		 
\end{comment}

==> codes/ch04_sssp_pregel.tex <==
\begin{algorithm}[h]
\compute{vertex, messages}
\Begin{
	changed $\leftarrow$ false\;
	\eIf{getSuperstep() = 0}{
		\tcc{first superstep: initialize values }
		\eIf{vertex.id = source}{
			vertex.distance $\leftarrow$ 0\;
			changed $\leftarrow$ true\;
		}{
			vertex.distance $\leftarrow$ $\infty$\;
		}
	}{
		minMsg $\leftarrow$ getMinumum(messages)\;
		\If{msg < vertex.distance}{
			\tcp{found smaller distance}
			vertex.distance $\leftarrow$ msg\;
			changed $\leftarrow$ true\;
		}
	}
	\If{changed}{
		\ForEach{edge $\in$ vertex.edges}{
			msg $\leftarrow$ vertex.distance + edge.weight\;
			\sendmsg(edge.targetVertex, msg)\;
		}
	}
	vertex.voteToHalt()\;
}
\caption{SSSP in Pregel}
\label{alg:sssp_pregel}
\end{algorithm}

\begin{comment}
if (getSuperstep() == 0) {
      setValue(new DoubleWritable(Double.MAX_VALUE));
    }
    double minDist = isSource() ? 0d : Double.MAX_VALUE;
    for (DoubleWritable message : messages) {
      minDist = Math.min(minDist, message.get());
    }
    if (LOG.isDebugEnabled()) {
      LOG.debug("Vertex " + getId() + " got minDist = " + minDist +
          " vertex value = " + getValue());
    }
    if (minDist < getValue().get()) {
      setValue(new DoubleWritable(minDist));
      for (Edge<LongWritable, FloatWritable> edge : getEdges()) {
        double distance = minDist + edge.getValue().get();
        if (LOG.isDebugEnabled()) {
          LOG.debug("Vertex " + getId() + " sent to " +
              edge.getTargetVertexId() + " = " + distance);
        }
        sendMessage(edge.getTargetVertexId(), new DoubleWritable(distance));
      }
    }
    voteToHalt();
\end{comment}

==> codes/clustering_approximate_gas.tex <==
\begin{algorithm}[h]
\SetKwFunction{gettotal}{getTotal}
\tcp{gather on all edges}
\gather{vertex, edge}
\Begin{
	\KwRet{[edge.otherVertex]}
}
\gathersum{list1, list2}
\Begin{
	append(list1, list2)\;
}
\apply{vertex, neighbours}
\Begin{
	vertex.neighbours = neighbours\;
	\If{vertex.numEdges > 1}{
		vertex.trials = getNumberOfTrials()\;
		\For{1 to trials}{
			u $\leftarrow$ randomNeighbour(vertex)\;
			\Repeat {u $\neq$ w} {
				w $\leftarrow$ randomNeighbour(vertex)\; 
			}
			\tcc{save vertex pair in temporary local data structure}
			selectedVertices.insert(u,w)\;
		}
	}
}
\tcp{scatter on all edges}
\scatter{vertex, edge}
\Begin{
	linksFound $\leftarrow$ 0\;
	u $\leftarrow$ edge.otherVertex\;
	\ForEach{w $\in$ selectedVertices.get(u)}{
		\If{u.hasNeighbour(w)}{
			linksFound $\leftarrow$ linksFound + 1\;
		}
	}
}
\gettotal{vertex}
\Begin{
	\eIf{vertex.numEdges > 1}{
		\If{calculate GLOBAL CC}{
			\KwRet{vertex.numEdges * (vertex.numEdges - 1)};
		}
		\ElseIf{calculate LOCAL AVG CC} {
				\KwRet{1};
		}
	}{
		\KwRet{0};
	}
}
\main{graph}
\Begin{
	total $\leftarrow$ mapReduceVertex(\gettotal)\;
	executeVertexProgram(graph)\;
	cc $\leftarrow$ mapReduceEdge(edge.linksFound) / mapReduceVertex(vertex.trials)\;
	
}
\caption{Approximate Clustering Coefficients in GAS}
\label{alg:gas_x}
\end{algorithm}

==> codes/clustering_approximate_giraph++.tex <==
\begin{algorithm}[h]
\SetKwFunction{getrandom}{getRandomVertex}
\SetKwData{Newrank}{newrank}
\compute{partition}
\Begin{
	linksFound $\leftarrow$ 0\;
	\If{getSuperstep() = 0 $\land$ mode = GLOBAL}{
		\tcc{only needed for global cc}
		localTotal $\leftarrow$ 0\;
		\ForEach{iv $\in$ getInternalVertices()}{
			\If{iv.numEdges > 1}{
				setAggregatorValue(TOTAL, iv.numEdges * (iv.numEdges - 1))\;
				localTotal $\leftarrow$ iv.numEdges * (iv.numEdges - 1)\;
			}
		}
	}
	\ElseIf{getSuperstep() = 1}{
		\eIf{mode = GLOBAL}{
			partitionSamples $\leftarrow$ s * localTotal / getAggregatorValue(TOTAL)\;
		}{
			partitionSamples $\leftarrow$ s * numPartitionVertices / numTotalVertices\;
		}
		\ForEach{i = 1..partitionSamples}{
			\tcc{for the local avg, choose random vertex from uniform distribution, for the global, the vertex probability increases with  p$_v$}
			v $\leftarrow$ \getrandom{v, mode}\;
			\eIf{v.numEdges < 2}{
				i - -\;
			}{
				u, w $\leftarrow$ getTwoDifferentNeighbours(v)\;
				\If{u is internal $\land$ u.hasNeighbour(w)}{
					linksFound++\;
				}
				\ElseIf{w is internal $\land$ w.hasNeighbour(u)}{
					linksFound++\;
				}
				\Else{
					\sendmsg{u, w}\;
				}
			}
		}
		setAggregatorValue(SAMPLES, partitionSamples)\;
	}
	\ElseIf{getSuperstep() = 2}{
		\ForEach{iv $\in$ getInternalVertices()}{
			\ForEach{msg $\in$ iv.getMessages()}{
				\If{iv.hasNeighbour(msg)}{
					linksFound++\;
				}
			}
		}
		setAggregatorValue(LINKS, linksFound)\;
	}
}
\mastercompute{}
\Begin{
	cc $\leftarrow$ getAggregatorValue(LINKS) / getAggregatorValue(SAMPLES)\;
}
\caption{Approximate Clustering Coefficients in Giraph++}
\label{alg:clustering_approximate_giraph++}
\end{algorithm}

==> codes/clustering_approximate_pregel.tex <==
\begin{algorithm}[h]
\SetKwFunction{getnumbertrials}{getNumberOfTrials}
\compute{vertex, messages}
\Begin{
	\If{getSuperstep() = 0 $\land$ vertex.numEdges > 1}{
	
		\If{calculate GLOBAL CC}{
			setAggregatorValue(TOTAL, vertex.numEdges * (vertex.numEdges - 1)\;
		}
		\ElseIf{calculate LOCAL AVG CC} {
			setAggregatorValue(TOTAL, 1)\;
		}
	}
	\ElseIf{getSuperstep() = 1}{
		trials = getNumberOfTrials()\;
		setAggregatorValue(TRIALS, trials)\;
		\For{1 to trials}{
			u $\leftarrow$ randomNeighbour(vertex)\;
			\Repeat {u $\neq$ w} {
				w $\leftarrow$ randomNeighbour(vertex)\; 
			}
			\sendmsg(u, w)\;
		}
	}
	\ElseIf{getSuperstep() = 2}{
		neighbourEdges $\leftarrow$ 0\;
		\For{$msg\in messages$}{
			\If{\msg $\in$ \vertex.edges}{
				neighbourEdges $\leftarrow$ neighbourEdges + 1\;
			}
		}
		
		setAggregatorValue(EDGES, neighbourEdges)\;
	}
}
\getnumbertrials{vertex}
\Begin{

	total $\leftarrow$ getAggregatorValue(TOTAL) / getAggregatorValue(TRIALS)\;
	\If{calculate GLOBAL CC}{
		numberOfTrials $\leftarrow$ TRIALS * vertex.degree * (vertex.degree - 1) / total\;
	}
	\ElseIf{calculate LOCAL AVG CC} {
		numberOfTrials $\leftarrow$ TRIALS / total\;
	}
	\If{numberOfTrials is not integer}{
		probability $\leftarrow$ numberOfTrials - roundDown(numberOfTrials)\;
		numberOfTrials $\leftarrow$ roundDown(numberOfTrials)\;
		\If{rand() < probability}{
			numberOfTrials++\;
		}
		
	}
	\KwRet{numberOfTrials}
}
\mastercompute{}
\Begin{
	approximation $\leftarrow$ getAggregatorValue(EDGES) / getAggregatorValue(TRIALS)\;
}
\caption{Approximate Clustering Coefficients in Pregel}
\label{alg:clustering_approximate_pregel}
\end{algorithm}

==> img/plots/cdlp_exectimes.tex <==
\pgfplotsset{cdlpchartl/.style={ 
       ybar,
       height=6.5cm,
       bar width=10pt,
       enlargelimits=0.15,
       legend style={at={(0.5,-0.15)},
         anchor=north,legend columns=-1},
       ylabel={Time in s},
       symbolic x coords={NetworKit, GraphLab},
       xtick=data,
       x=1.6cm,
       nodes near coords,
       nodes near coords align={vertical},
       area legend,
       enlarge x limits=0.5,
       x post scale=1.5,
     cycle list name=nodescolors,
    } 
}
\pgfplotsset{cdlpchartr/.style={ 
       ybar,
       height=6.5cm,
       bar width=10pt,
       enlargelimits=0.15,
       legend style={at={(0.5,-0.15)},
         anchor=north,legend columns=-1},
       ylabel={Time in s},
                symbolic x coords={Giraph, Giraph++, Flink},
       xtick=data,
       x=1.6cm,
       nodes near coords,
       nodes near coords align={vertical},
       area legend,
      enlarge x limits=0.3,
       x post scale=1.5,
     cycle list name=nodescolors,
    } 
}
\begin{figure}[H]
  \centering
\begin{minipage}{.43\textwidth}
 \begin{tikzpicture}
    \node[text width=5cm] (title) at (2.6, 5.4) {\graFlickrEdges};
   \begin{axis}[cdlpchartl]
   \addplot coordinates {(NetworKit,0.5) (GraphLab,1.4)};
   \addplot coordinates { 				(GraphLab,2) };
   \addplot coordinates {				(GraphLab,2) };
   \addplot coordinates { 				(GraphLab,3) };
   %\legend{1,2,4,8}
   \end{axis}
   \end{tikzpicture}
\end{minipage}
\begin{minipage}{.56\textwidth}
   \begin{tikzpicture}
     \begin{axis}[cdlpchartr]
         \node[text width=5cm] (title) at (2.6, 5.4) { .};
		\addplot coordinates {(Giraph,159) (Giraph++,) (Flink,122)};
		\addplot coordinates {(Giraph,149) (Giraph++,) (Flink,88)};
		\addplot coordinates {(Giraph,80) (Giraph++,64) (Flink,65)};
		\addplot coordinates {(Giraph,69) (Giraph++,348) (Flink,51)};
	     %\legend{1,2,4,8}
     \end{axis}
     
     \end{tikzpicture}
    \end{minipage}%
    
    
    \begin{minipage}{.43\textwidth}
     \begin{tikzpicture}
        \begin{axis}[cdlpchartl]
       \addplot coordinates {(NetworKit,24.8) (GraphLab,99.3)};
       \addplot coordinates { 				(GraphLab,96) };
       \addplot coordinates {				(GraphLab,52.3) };
       \addplot coordinates { 				(GraphLab,50.3) };
       %\legend{1,2,4,8}
       \end{axis}
       \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{.56\textwidth}
       \begin{tikzpicture}
            \begin{axis}[cdlpchartr]
    		\addplot coordinates {(Giraph,1462) (Giraph++,1) (Flink,1)};
    		\addplot coordinates {(Giraph,1318) (Giraph++,1) (Flink,1)};
    		\addplot coordinates {(Giraph,647.95) (Giraph++,1) (Flink,1)};
    		\addplot coordinates {(Giraph,1) (Giraph++,1) (Flink,1)};
    	     %\legend{1,2,4,8}
         \end{axis}
         
         \end{tikzpicture}
        \end{minipage}%

\begin{minipage}{.43\textwidth}
 \begin{tikzpicture}
    \begin{axis}[cdlpchartl]
          \addplot coordinates {(NetworKit,16.68) (GraphLab,48.6)};
          \addplot coordinates { 				(GraphLab,67.74) };
          \addplot coordinates {				(GraphLab,41.48) };
          \addplot coordinates { 				(GraphLab,0) };
   \legend{1,2,4,8}
   \end{axis}
   \end{tikzpicture}
\end{minipage}
\begin{minipage}{.56\textwidth}
   \begin{tikzpicture}
        \begin{axis}[cdlpchartr]
		\addplot coordinates {(Giraph,698)};
		\addplot coordinates {(Giraph,633) };
		\addplot coordinates {(Giraph,322) };
		\addplot coordinates {(Giraph,233) (Giraph++,1411)};
	     \legend{1,2,4,8}
     \end{axis}
     
     \end{tikzpicture}
    \end{minipage}%
  
  \begin{minipage}{.43\textwidth}
   \begin{tikzpicture}
      \begin{axis}[cdlpchartl]
            \addplot coordinates { 				(GraphLab,1342) };
     \legend{1,2,4,8}
     \end{axis}
     \end{tikzpicture}
  \end{minipage}
\begin{minipage}{.56\textwidth}
 \begin{tikzpicture}
      \begin{axis}[cdlpchartr]
 		\addplot coordinates {(Giraph,1958)};
    \legend{1,2,4,8}
   \end{axis}
        \end{tikzpicture}
       \end{minipage}
\begin{minipage}{.43\textwidth}
 \begin{tikzpicture}
    \begin{axis}[cdlpchartl]
          \addplot coordinates {(NetworKit,17.16) };
          \addplot coordinates { 				(GraphLab,140) };
   \legend{1,2,4,8}
   \end{axis}
   \end{tikzpicture}
\end{minipage}
\begin{minipage}{.56\textwidth}
   \begin{tikzpicture}
        \begin{axis}[cdlpchartr]
		\addplot coordinates {(Giraph,993) (Giraph++,1856)};
	     \legend{1,2,4,8}
     \end{axis}
     
     \end{tikzpicture}
    \end{minipage}%
	\caption[Community Detection Execution times]{Execution times of the Community Detection Label Propagation for the \graOrkut (top) and \graLiveU (bottom) graph on 1,2,4 and 8 nodes. The left graph shows the the asynchronous executions in NetworKit and GraphLab, the right graph the synchronous executions which do not converge, for 40 iterations.}
	\label{fig:perf_cc_orkut}   
\end{figure}


==> img/plots/concomp_iterations_g++.tex <==
\pgfplotsset{mychart1/.style={ 
      ybar,	
      bar width=10pt,
      enlargelimits=0.20,
      legend style={at={(0.5,-0.15)},
        anchor=north,legend columns=-1},
      ylabel={number of supersteps},
      symbolic x coords={1,2,4,8},
      xtick=data,
      xtick pos=left,
      x=1.05cm,
      %nodes near coords,
      %nodes near coords align={vertical},
      area legend,
      cycle list name=GiGpColors,
    } 
}

\begin{figure}[H]
  \centering
  \begin{minipage}{.36\textwidth}
 \centering
  \begin{tikzpicture}
  \begin{axis}[mychart1, title={\graFlickrLinks},
      ]
  \addplot coordinates {(1,15) (2,15) 	(4,15) (8,15)};
  \addplot coordinates {(1,5) (2,	10) 	(4,10) (8,10)};
  \legend{Giraph, Giraph++}
  \end{axis}
  \end{tikzpicture}

  \end{minipage}%
\begin{minipage}{.32\textwidth}
   \centering
    \begin{tikzpicture}
    \begin{axis}[mychart1, title={\graLiveU},
        ]
          \addplot coordinates {(1,15) (2,15) 	(4,15) (8,15)};
          \addplot coordinates {(1,6) (2,	6) 	(4,8) (8,12)};
          \legend{Giraph, Giraph++}
    \end{axis}
    \end{tikzpicture}
    \end{minipage}%
\begin{minipage}{.3\textwidth}
   \centering
    \begin{tikzpicture}
    \begin{axis}[
        mychart1, title={\graOrkut},
        ]
      \addplot coordinates {(1,8) (2,8) 	(4,8) (8,8)};
      \addplot coordinates {(1,5) (2,	5) 	(4,5) (8,5)};
      \legend{Giraph, Giraph++}
    \end{axis}
    \end{tikzpicture}
    \end{minipage}  
    \caption[Number of supersteps in Giraph++]{Number of supersteps in the Connected Components algorithm in Giraph and Giraph++.}
    \label{fig:iterations_g++}
\end{figure}

==> img/plots/exact_clustering_times.tex <==

\pgfplotsset{mychartex/.style={ 
        ybar, 
        height=5.5cm,
        log ticks with fixed point, point meta=rawy,
        bar width=11pt, 
        enlargelimits=0.15,
        legend style={at={(0.5,-0.15)},
        anchor=north,legend columns=-1},
        ylabel={Time in s},
              symbolic x coords={NetworKit, GraphLab, Giraph},
      xtick=data, x=2.8cm, nodes near coords, nodes near coords align={vertical},
      area legend,
      every node near coord/.append style={font=\small},
      		cycle list name=nodescolors,
    } 
}

\begin{figure}[H]
  \centering
 	\begin{tikzpicture}
      \begin{axis}[
      	  mychartex,
      	  ymode=log, 
          ]
      \addplot coordinates {(NetworKit,55) (GraphLab,183) (Giraph,789)};
      \addplot coordinates {(GraphLab,154) (Giraph,760)};
      \addplot coordinates {(GraphLab,61) (Giraph,410)};
      \addplot coordinates { (GraphLab,34) (Giraph,219)};
      \legend{1,2,4,8}
      \end{axis}
      \end{tikzpicture}
            \caption[Clustering Coefficients execution times]{Execution times of \algClEx for the \graFlickrEdges graph}
          \label{fig:clustering_exact}
\end{figure}

==> img/plots/pagerank_weak.tex <==
\begin{figure}[H]

  \centering
  \resizebox{.5\textwidth}{!}{
  %\begin{minipage}{.9\textwidth}
 \centering
  \begin{tikzpicture}
  \begin{axis}[weakchart]
  \addplot coordinates {(1,77) (2,120) (4,194) (8,207)};
  \addplot coordinates {(1,137) (2,148) (4,152) (8,176)};
  \addplot coordinates {(1,97) (2,107) (4,149) (8,169)};
  \legend{GraphLab, Giraph, Flink}
  \end{axis}
  \end{tikzpicture}

  %\end{minipage}
  }
    \caption[PageRank weak scaling]{Weak scaling of PageRank with generated data sets of 16 million edges per node}
    \label{fig:pagerank_weak}
\end{figure}

==> img/plots/sampling_clustering_times.tex <==
\pgfplotsset{mychartex/.style={ 
	mychart,
        height=6cm,
        bar width=14pt, 
      symbolic x coords={NetworKit, GraphLab, Giraph},
    } 
}

\begin{figure}[H]
  \centering
 	\begin{tikzpicture}
 	 \node[text width=5cm] (title) at (2.9,3.5) {\graFlickrEdges};
      \begin{axis}[
      	  mychart,
      	  ymode=log, 
          ]
      \addplot coordinates {(NetworKit,0.09) (GraphLab,1.35) 	(Giraph,16.7) (Giraph++,) (Flink,20)};
      \addplot coordinates { 				(GraphLab,3.75) 	(Giraph,14.8) (Giraph++,) (Flink,28)};
      \addplot coordinates {				(GraphLab,2.2) 	(Giraph,12.2) (Giraph++,23.7) (Flink,26)};
      \addplot coordinates { 				(GraphLab,2.2) 		(Giraph,5.4) (Giraph++,24.1) (Flink,2)};
      \end{axis}
      \end{tikzpicture}
      \label{fig:perf_clustering_sampling}
      \caption[Clustering Coeffcients apprxoimation execution times]{Execution times for the Clustering Cofficient aproximation (average local approximation, 100.000 samples)}
\end{figure}


==> plots/async_vs_sync_time.tex <==
\begin{multicols}{2}
\begin{figure*}[h]
  \centering
%  \begin{minipage}{.30\textwidth}
% \centering
\subfloat[][]{
  \begin{tikzpicture}
  \begin{axis}[
      ybar,
      bar width=10pt,
      enlargelimits=0.20,
      legend style={at={(0.5,-0.15)},
        anchor=north,legend columns=-1},
      ylabel={Time in s},
      symbolic x coords={1,2,4,8},
      xtick=data,
      x=1.05cm,
      nodes near coords,
      nodes near coords align={vertical},
      area legend,
      ]
  \addplot coordinates {(1,27) (2,26) 	(4,23) (8,21.3)};
  \addplot coordinates {(1,24) (2,	45) 	(4,34) (8,26.9)};
  \legend{synch, asynch}
  \end{axis}
  \end{tikzpicture}
 }
%
\subfloat[][]{
    \begin{tikzpicture}
    \begin{axis}[
        ybar,
        bar width=10pt,
        enlargelimits=0.20,
        legend style={at={(0.5,-0.15)},
          anchor=north,legend columns=-1},
        ylabel={},
        symbolic x coords={1,2,4,8},
        xtick=data,
        x=1.05cm,
        nodes near coords,
        nodes near coords align={vertical},
        area legend,
        ]
    \addplot coordinates {(1,25) (2,24) 	(4,21) (8,17.6)};
    \addplot coordinates {(1,44) (2,	57) 	(4,45) (8,33.01)};
    \legend{synch, asynch}
    \end{axis}
    \end{tikzpicture}
 }


%  \end{minipage}%
%\begin{minipage}{.30\textwidth}
   \centering
%    \end{minipage}%
%\begin{minipage}{.30\textwidth}
   \centering
    \begin{tikzpicture}
    \begin{axis}[
        ybar,
        bar width=10pt,
        enlargelimits=0.20,
        legend style={at={(0.5,-0.15)},
          anchor=north,legend columns=-1},
        ylabel={},
        symbolic x coords={1,2,4,8},
        xtick=data,
        x=1.05cm,
        nodes near coords,
        nodes near coords align={vertical},
        area legend,
        ]
    \addplot coordinates {(1,37) (2,27) 	(4,9) (8,9.3)};
    \addplot coordinates {(1,40) (2,33) 	(4,11) (8,12.3)};
    \legend{synch, asynch}
    \end{axis}
    \end{tikzpicture}
%    \end{minipage}  
    \caption[Execution time and vertex updates in asynchronous and synchronous execution]{Comparison of Graphlab's synchronous and asynchronous execution for Connected Components, message based Connected Components and PageRank (from left to right) on the Livejournal graph. The top diagram shows the number of updated vertices, the bottom one the algorithm exection time.}
    \label{fig:asnyc_vs_sync}
\end{figure*}
\end{multicols}

==> plots/async_vs_sync_updates.tex <==
\begin{multicols}{2}
\begin{figure*}[h]
  \centering
%  \begin{minipage}{.30\textwidth}
 \centering
  \begin{tikzpicture}
  \begin{axis}[
  	  title={\algcc},
      ybar,	
      bar width=10pt,
      enlargelimits=0.20,
      legend style={at={(0.5,-0.15)},
        anchor=north,legend columns=-1},
      ylabel={vertex updates in millions},
      symbolic x coords={1,2,4,8},
      xtick=data,
      xtick pos=left,
      x=1.05cm,
      %nodes near coords,
      %nodes near coords align={vertical},
      area legend,
      ]
  \addplot coordinates {(1,23.926633) (2,23.926633) 	(4,23.926633) (8,23.926633)};
  \addplot coordinates {(1,7.183493) (2,	12.030581) 	(4,12.358260) (8,12.661198)};
  \legend{synch, asynch}
  \end{axis}
  \end{tikzpicture}

%  \end{minipage}%
%\begin{minipage}{.30\textwidth}
   \centering
    \begin{tikzpicture}
    \begin{axis}[
      	title={\algccm},
      	%title style={yshift=-1.5ex},
        ybar,
        bar width=10pt,
        enlargelimits=0.20,
        legend style={at={(0.5,-0.15)},
          anchor=north,legend columns=-1},
        ylabel={},
        symbolic x coords={1,2,4,8},
        xtick=data,
        x=1.05cm,
        %nodes near coords,
        %nodes near coords align={vertical},
        area legend,
        ]
    \addplot coordinates {(1,29.125113) (2,29.125113) 	(4,29.125113) (8,29.125113)};
    \addplot coordinates {(1,12.661962) (2,	18.300533) 	(4,19.186572) (8,17.229823)};
    \legend{synch, asynch}
    \end{axis}
    \end{tikzpicture}
%    \end{minipage}%
%\begin{minipage}{.30\textwidth}
   \centering
    \begin{tikzpicture}
    \begin{axis}[
        ybar,
        title={\algpr},
        bar width=10pt,
        enlargelimits=0.20,
        legend style={at={(0.5,-0.15)},
          anchor=north,legend columns=-1},
        ylabel={},
        symbolic x coords={1,2,4,8},
        xtick=data,
        x=1.05cm,
        %nodes near coords,
        %nodes near coords align={vertical},
        area legend,
        ]
    \addplot coordinates {(1,10.699778) (2,10.699778) 	(4,10.699778) (8,10.699778)};
    \addplot coordinates {(1,5.577698) (2,5.636313) 	(4,5.653858) (8,5.631472)};
    \legend{synch, asynch}
    \end{axis}
    \end{tikzpicture}
%    \end{minipage}  
\end{figure*}
\end{multicols}

==> plots/graphlaboptions_time.tex <==
\begin{multicols}{2}
\begin{figure*}[h]
  \centering
%\begin{minipage}[t]{.46\textwidth}
 \begin{tikzpicture}
   \begin{axis}[
   		title={\graLiveU, sync},
       ybar,
       bar width=12pt,
       enlarge y limits={upper,value=0.2},
      legend style={at={(1.03,-1.43)},
        anchor=north,legend columns=-1},
       legend style={overlay},
       ylabel={Time in s},
       symbolic x coords={1,2,4,8},
       xtick=data,
       x=1.2cm,
       nodes near coords,
       nodes near coords align={vertical},
       area legend,
       enlarge x limits=0.2,
       x post scale=1.5,
       every node near coord/.append style={font=\small,rotate=90,anchor=west}
       ]
       
        \addplot coordinates {(1,61.7) (2,41) (4, 29.2) (8,1)};
        \addplot coordinates {(1, 55.6) (2,37.5) (4, 25.5) (8,17.6)};
        \addplot coordinates {(1,52.2) (2,37) (4, 	26.9) (8,21.03)};
           \legend{Standard, Message API, Delta Caching}
        
   \end{axis}
   \end{tikzpicture}
%\end{minipage}
%\begin{minipage}[t]{.46\textwidth}
   \begin{tikzpicture}
     \begin{axis}[
        	title={\graOrkut, sync},
            ybar,
            bar width=12pt,
            enlarge y limits={upper,value=0.2},
            legend style={at={(0.5,-0.15)},
              anchor=north,legend columns=-1},
            symbolic x coords={1,2,4,8},
            xtick=data,
            x=1.2cm,
            nodes near coords,
            nodes near coords align={vertical},
            area legend,
            enlarge x limits=0.2,
            x post scale=1.5,
            every node near coord/.append style={font=\small,rotate=90,anchor=west}
         ]
               
         \addplot coordinates {(1,27.4) (2,26.0) (4, 23.2) (8,1)};
	         \addplot coordinates {(1, 24.6) (2,24) (4, 20.9) (8,19.33)};
         \addplot coordinates {(1,24.6) (2,24.5) (4, 	23.9) (8,23.7)};
     \end{axis}
     \end{tikzpicture}
%    \end{minipage}
%    
%\begin{minipage}[t]{.46\textwidth}
 \begin{tikzpicture}
   \begin{axis}[
       ybar,
        title={\graLiveU, async},
       bar width=12pt,
       enlarge y limits={upper,value=0.2},
       legend style={at={(1,-0.17)},
         anchor=north,legend columns=-1},
                       legend style={overlay},
       ylabel={Time in s},
       symbolic x coords={1,2,4,8},
       xtick=data,
       x=1.2cm,
       nodes near coords,
       nodes near coords align={vertical},
       area legend,
       enlarge x limits=0.2,
       x post scale=1.5,
       every node near coord/.append style={font=\small,rotate=90,anchor=west}
       ]
       
        \addplot coordinates {(1,50.2) (2,60.2) (4, 40.2) (8,26.9)};
        \addplot coordinates {(1, 79.3) (2,59.4) (4,47.2) (8,33)};
   \end{axis}
   \end{tikzpicture}
%\end{minipage}
%\begin{minipage}[t][][t]{.46\textwidth}
   \begin{tikzpicture}
     \begin{axis}[
            ybar,
            title={\graOrkut, async},
            bar width=12pt,
            enlarge y limits={upper,value=0.2},
            legend style={at={(0.5,-0.15)},
              anchor=north,legend columns=-1},
            symbolic x coords={1,2,4,8},
            xtick=data,
            x=1.2cm,
            nodes near coords,
            nodes near coords align={vertical},
            area legend,
            enlarge x limits=0.2,
            x post scale=1.5,
            every node near coord/.append style={font=\small,rotate=90,anchor=west}
         ]
                 \addplot coordinates {(1,24.4) (2,45) (4, 34.3) (8,27.7)};
                 \addplot coordinates {(1, 44.3) (2,56.8) (4,44.6) (8,43.4)};
     \end{axis}
     \end{tikzpicture}
%    \end{minipage}%
    	\vspace{.9cm}
	\caption[GraphLab's messaging and delta caching performance]{GraphLab's messaging and delta caching performance: Execution times of the standard, message based and delta caching versions of \algcc for the livejournal-links graph (left) and the orkut-links graph (right) in synchronous and aysynchronous modes}
	\label{fig:graphlab_options}    
\end{figure*}
\end{multicols}
